Autonomous Local Catalog Maintenance of Close Proximity Satellite Systems on Closed Natural Motion Trajectories

To enable space mission sets like on-orbit servicing and manufacturing, agents in close proximity maybe operating too close to yield resolved localization solutions to operators from ground sensors. This leads to a requirement on the systems need to maintain a catalog of their local neighborhood, however, this may impose a large burden on each agent by requiring updating and maintenance of this catalog at each node. To alleviate this burden, this paper considers the case of a single satellite agent (a chief) updating a single catalog. More specifically, we consider the case of numerous satellite deputy agents in a local neighborhood of a chief, the goal of the chief satellite is to maintain and update a catalog of all agents within this neighborhood through onboard measurements. We consider the agents having relative translational and attitude motion dynamics between the chief and deputy, with the chief centered at the origin of the frame. We provide an end-to-end solution of the this problem through providing both a supervisory control method coupled with a Bayesian Filter that propagates the belief state and provides the catalog solutions to the supervisor. The goal of the supervisory controller is to determine which agent to look at and at which times while adhering to constraints of the chief satellite. We provide a numerical validation to this problem with three agents.

==> sections/CutContent.tex <==
\section{Cut Content}
\label{sec:cut_content}
\alex{In no particular order, this is material removed from the abstract and placed into the full paper.}





==> sections/old_problem.tex <==
\section{Preliminaries}
Let $\reals$ denote the set of all real numbers.
A frame for an $n$-dimensional space is defined by $n$ orthonormal vectors $\hat{\inertialframe}_i$, $i \in [1,n]$.
In this paper, we work with spaces where $n=3$. The Lie Group $\soThree$ is the set of all real invertible $3 \times 3$ matrices that are orthogonal with determinant $1$, in this work referred to as \textit{rotation matrices} $\rotmat{}{} \in \SOThree:$
$$\SOThree := \{\rotmat{}{} \in \reals^{3 \times 3} \ | \ (\rotmat{}{})^{T}\rotmat{}{} = \idMat{3}, \det[\rotmat{}{}] = 1\}$$
Given two coordinate frames $\A$ and $\B$, the rotation of vector $\deputyState^{\A} \in \A$ to $\deputyState^{\B} \in \B$ is denoted by $\rotmat{\A}{\B}$,
that is, $\deputyState^{\B} = \rotmat{\A}{\B} \deputyState^{\A}$.
Additionally, we will be dealing with angular velocities.
Given three frames $\A$, $\B$, and $\C$, the angular velocity of $\B$ relative to $\A$ as measured in frame $\C$ is denoted by 
$\angularvel{\A}{\B}{\C}$. For a vector $\textbf{a} := (a_1 \ a_2 \ a_3)^{\top} \in \reals^3$, the cross product operator $\skewMat{\cdot} : \reals^{3} \to \soThree$:
\begin{equation}
\skewMat{\textbf{a}} =
\begin{pmatrix} 
0 & -a_3 & a_2 \\
a_3 & 0 & -a_1 \\
-a_2 & a_1 & 0
\end{pmatrix}
\label{eq:skewmat}
\end{equation}
If $\textbf{b} \in \reals^3$, then the cross-product $\textbf{c} = \textbf{a} \times \textbf{b}$ can be written $\textbf{c} = \skewMat{\textbf{a}}\textbf{b} = -\skewMat{\textbf{b}}\textbf{a}$. Here, the Lie algebra $\soThree$ is the set of all real $3 \times 3$ skew-symmetric matrices and is the tangent space of $\SOThree$ at the identity $\idMat{3}$:
$$\soThree := \{\skewMat{\textbf{a}}^{T} = -\skewMat{\textbf{a}} \ | \ \textbf{a} \in \reals^3\}$$
 For a vector $\textbf{a} \in \reals^3$, the $\mathcal{L}^2$ norm operator is defined as $\norm{\textbf{a}} := \sqrt{\textbf{a}^{\top} \textbf{a}}$. A multivariate Gaussian distribution of an $n$-dimensional random variable is parameterized by a mean vector $\hat{\deputyState} \in \reals^n$ and a symmetric, positive semidefinite covariance matrix $\deputyUncertainty \in \reals^{n \times n}$.
Next, we specify a mapping between the vector $\deputyState$ in Cartesian space to the azimuth-elevation space $g(\deputyState) : \reals^{3} \to \sphere^{2}$ 
\begin{equation}
    g(\deputyState) = 
    \begin{bmatrix}
    \tan^{-1}(\frac{s_{2}}{s_{1}})\\
    \sin^{-1}(s_{3})
    \end{bmatrix}
\end{equation}
where $s=\frac{\deputyState}{\norm{\deputyState}}$ and $\sphere^2$ is the unit sphere with angular coordinates $\Azimuth \in [-\pi, \pi]$ and $\Elevation \in [-\frac{\pi}{2}, \frac{\pi}{2})$ by astronomical convention. In particular, this mapping is used to project the natural motion trajectories of the deputies onto the local attitude space $(\Azimuth, \Elevation)$ of the chief.

\subsection{Local Catalog Maintenance} 
To maintain the local catalog, a chief satellite equipped with a sensor and on-board estimating capabilities must track and maintain the states of several deputy satellites. The inherent uncertainties of the deputies' states are characterized via some stochastic representation, generally through a state probability distribution. The uncertainty attached to this so-called ``belief state" can be quantified and ideally guaranteed to lie underneath a predefined bound, which is the root of the maintenance problem. As the time since the last observation of a deputy increases, the parameterization of the deputy's belief state uncertainty (e.g. the state covariance matrix for a Gaussian representation) grows accordingly.
% uncertainty in that deputy's state increases.
Additionally, the chief cannot observe the states of all the deputies simultaneously.
Thus, the problem that we are addressing is the design of a controller for the chief such that the states of all the deputy satellites are known within some certainty. The local catalog maintenance problem is formalized in this section.

\subsection{Model Predictive Control}
\label{sec:MPC}
\alex{Alex will do this.}


\subsection{Relative Motion Dynamics}

Consider the chief spacecraft in a circular orbit centered on the earth.
The chief does not have thrusters for translational motion, but can rotate about its center of mass in the circular orbit using reaction wheels. Thus, the frames we are concerned with are Hill's frame $\hillsframe$,
the inertial frame $\inertialframe$, and the chief body frame $\bodyframe$, as depicted in Figure \ref{fig:frames}. Note that both the Hill's frame $\hillsframe$ and the body-fixed frame $\bodyframe$ rotate with respect to the inertial frame.

\begin{figure}[ht!]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \begin{tikzpicture}
        \draw[thick, dotted] (0,0) ellipse (3 and 1);
        \draw[rotate=60, dashed] (0,0) ellipse (3 and 1);
        
        \draw[fill=black!40] (0,0) circle (0.75);
        \draw[fill=white] (1.5,2.5) circle (0.2);
        \draw[fill=white] (3,0) circle (0.2);
        
        \draw[-stealth] (0,0) -- (3,0);
        \draw[-stealth] (0,0) -- (1.5,2.5);
        \draw[-stealth] (3,0) -- (1.5,2.5);
        
        \draw[-stealth,thick] (3,0) -- (4,0);
        \draw[-stealth,thick] (3,0) -- (3,1);
        \draw[-stealth,thick] (3,0) -- (3.7,0.7);
        
        \node at (4.2,0) {$\hat{x}_{\hillsframe}$};
        \node at (3.9,0.9) {$\hat{y}_{\hillsframe}$};
        \node at (3,1.2) {$\hat{z}_{\hillsframe}$};
        
        \node at (1.6,-0.3) {$\overrightarrow{r}_{c}$};
        \node at (0.4,1.3) {$\overrightarrow{r}_{d}$};
        \node at (2.7,2) {$\state \restr \reals^3$};
        
        \node at (3.5,-0.4) {Chief};
        \node at (1.5,3) {Deputy};
    \end{tikzpicture}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \begin{tikzpicture}
        \draw[thick, ->] (0,0) -- (2,0);
        \draw[thick, ->] (0,0) -- (0,2);
        \draw[thick, ->] (0,0) -- (1.4,1.4);
        
        \draw[rotate=20, dotted, ->] (0,0) -- (2,0);
        \draw[rotate=20, dotted, ->] (0,0) -- (0,2);
        \draw[rotate=20, dotted, ->] (0,0) -- (1.4,1.4);
        
        \draw[rotate=20] (-0.5,0.5) -- (0.5,0.5) -- (0.5,-0.5) -- (-0.5,-0.5) -- (-0.5,0.5) -- (-0.3,0.7) -- (0.7,0.7) -- (0.7,-0.3) -- (0.5,-0.5);
        
        \node at (0,-1) {Chief};
        \node at (2.3,0) {$\hat{x}_{\hillsframe}$};
        \node at (0,2.3) {$\hat{z}_{\hillsframe}$};
        \node at (1.7,1.7) {$\hat{y}_{\hillsframe}$};
        
        \node at (0,-1) {Chief};
        \node at (2,0.9) {$\hat{x}_{\bodyframe}$};
        \node at (-1,2) {$\hat{z}_{\bodyframe}$};
        \node at (0.8,2) {$\hat{y}_{\bodyframe}$};
    \end{tikzpicture}
    \end{subfigure}
    \caption{Left: Hill's frame $\hillsframe := \{\hat{x}_{\hillsframe}, \hat{y}_{\hillsframe}, \hat{z}_{\hillsframe}\}$. Here, $\overrightarrow{r}_c$ is the vector pointing from the center of the earth to the chief and $\overrightarrow{r}_d$ is the vector pointing from the center of the earth to a deputy. The frame is affixed to the chief satellite, and defined by the unit vectors (i) $\hat{x}_{\hillsframe}$ pointing in the direction of $\overrightarrow{r}_c$, (ii) $\hat{z}_{\hillsframe}$ pointing in the direction of the chief's angular momentum relative to the earth, and (iii) $\hat{y}_{\hillsframe} = \skewMat{\hat{x}_{\hillsframe}}\hat{z}_{\hillsframe}$.
    % {\color{green} Why are you using a $\hat {\mathcal H}$ as the reference frame? This is overkill unless you are out of symbols, just use $(i,j,k)$ or something. Please keep it simple.} 
    Right: Chief body frame $\bodyframe$ and Hill's frame $\hillsframe$. Note that $\bodyframe$ and $\hillsframe$ share an origin.
    }
    \label{fig:frames}
\end{figure}

The chief is tasked with maintaining the states of $m$ deputies.
The translational dynamics of the deputies in $\hillsframe$ are described by the Clohessy-Wiltshire equations.
% shown in~\eqref{eq:cw_equations} with
The state of a deputy $i \in [1,m]$ is given by $\deputyState_i = [r^i_x \ r^i_y \ r^i_z \ \dot{r}^i_x \ \dot{r}^i_y \ \dot{r}^i_z]^{\top}$, where
$r^i_x$, $r^i_y$, and $r^i_z$ are the $x_{\hillsframe}$-, $y_{\hillsframe}$-, $z_{\hillsframe}$-positions of deputy $i$ in $\hillsframe$ respectively.
The Clohessy-Wiltshire equations can be written in state-space form as in~\eqref{eq:A-matrix}.
% $\dot{\deputyState}_i = \deputyStateMat \deputyState_i$.
% where the state of each deputy $i \in [1, n]$ is given by
% $\deputyState_i = [r_x \ r_y \ r_z \ \dot{r}_x \ \dot{r}_y \ \dot{r}_z]$, and $\deputyStateMat$ is given in~\eqref{eq:A-matrix}.

% \begin{gather}
%     \Ddot{r}_x = 2 \meanmotion \dot{r}_y + 3 \meanmotion^2 r_x \nonumber \\
%     \Ddot{r}_y = 2 \meanmotion \dot{r}_x  \nonumber \\
%     \Ddot{r}_z = - \meanmotion^2 r_z
%     \label{eq:cw_equations}
% \end{gather}

\begin{equation}
    \dot{\deputyState}_i = \begin{bmatrix}
        \\
        & \zeroMat{3}{3} & & \idMat{3} & \\
        \\
        3 \meanmotion^2 & 0 & 0 & 0 & 2 \meanmotion & 0 \\
        0 & 0 & 0 & 2 \meanmotion & 0 & 0 \\
        0 & 0 & -\meanmotion^2 & 0 & 0 & 0
    \end{bmatrix} \deputyState_i
    \label{eq:A-matrix}
\end{equation}

Each deputy's relative state trajectory $\deputyState_i$ is uncontrolled and evolves under the following assumptions:
(i) $\dot{r}^i_y = -2 \meanmotion r^i_x$ and
(ii) $\dot{r}^i_x = \frac{1}{2} \meanmotion r^i_y$.
Condition (i) ensures that each deputy is in a periodic, closed natural motion trajectory (NMT).
There are three types of NMTs:
a stationary point, a line segment, and a closed ellipse.
Each NMT satisfies the requirement $\dot{r}_y = -2 \meanmotion r_x$, as well as the following:
(i) a stationary point has the requirements $r_x = r_z = \dot{r}_x = \dot{r}_z = 0$,
(ii) a line segment has the requirement $r_x = \dot{r}_x = 0$, $r_z = c \sin(\Psi)$, and $\dot{r}_z  = \meanmotion c \cos(\Psi)$ where $c$ is the length of the segment in $z_{\hillsframe}$-direction and $\Psi$ is the initial angle between the chief and the $x_{\hillsframe} y_{\hillsframe}$-plane, and
(iii) a closed ellipse centered at the CW origin has the requirement $\dot{r}_x = \frac{1}{2} \meanmotion r_y$.
Examples of these NMTs can be seen in Figure~\ref{fig:nmt-examples}.

\begin{figure}[h!]
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/elliptical_nmt.eps}
         \caption{Elliptical}
         \label{fig: nmt_types_elliptical}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/periodic_line_nmt.eps}
         \caption{Periodic Line Segment}
         \label{fig: nmt_types_line}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/stationary_nmt.eps}
         \caption{Stationary}
         \label{fig: nmt_types_stationary}
     \end{subfigure}
        \caption{Examples of Closed Natural Motion Trajectories}
        \label{fig:nmt-examples}
\end{figure}
Condition (ii) ensures that the relative state trajectory in the $r^i_x-r^i_y$ plane traces out a stationary $2 \times 1$ ellipse centered about the CW frame origin \cite{shepperd1991constant}. As the periodic positional trajectories of the deputies can be mapped with relative distance $r^{i} := \sqrt{(r^{i}_x)^2 + (r^{i}_y)^2 + (r^{i}_z)^2}$ and local $(\Azimuth^i, \Elevation^i)$ coordinates about the constantly rotating $\hillsframe$ frame, the rotation matrix $\rotmat{\hillsframe}{\inertialframe}$ maps these positions into the inertial $\inertialframe$ frame and informs the attitudinal guidance of the chief. 
% \begin{align}
% \label{eq:NMT_def}
%     \dot{r}_y &= -2 \meanmotion r_x \\
% \label{eq:ellipse_def}
%     \dot{r}_x &= \frac{1}{2} \meanmotion r_y
% \end{align}
% where condition \eqref{eq:NMT_def} ensures that each deputy is in a periodic, closed natural motion trajectory (NMT) while condition \eqref{eq:ellipse_def} ensures that the relative state trajectory in the $r_x-r_y$ plane traces out a stationary $2 \times 1$ ellipse centered about the CW frame origin \cite{shepperd1991constant}.


\begin{comment}
The rotation matrix $\rotmat{\inertialframe}{\hillsframe}$ from the inertial frame to Hill's frame can be computed given the position and orbital angular velocity of the chief, both in $\inertialframe$. The time rate change of any rotation matrix $\rotmat{\B}{\A}$ is given as
\begin{align}
\label{eq:rotation_velocity_a}
\dotrotmat{\B}{\A} &= \rotmat{\B}{\A}\skewMat{\angularvel{\A}{\B}{\B}} \\
\label{eq:rotation_velocity_b}
\dotrotmat{\B}{\A} &= \skewMat{\angularvel{\A}{\B}{\A}}\rotmat{\B}{\A}.
\end{align}
\end{comment}

\subsection{Chief Attitude Dynamics}

The rotation kinematics for the chief's body-fixed frame $\bodyframe$ are shown in~\eqref{eq:rotation_velocity_b}.
Assuming that the chief spacecraft can be modeled as a rigid body and has an inertia matrix $\chiefInertia$ as measured in the body-fixed frame, the application of Euler's second law of motion gives the attitude dynamics in~\eqref{eq:deputy_slew}, where $\chiefInput^{\bodyframe} \in \reals^3$ is the torque input for the chief as measured in the body frame about its center of mass.
% 
\begin{gather}
\label{eq:rotation_velocity_b}
\dotrotmat{\bodyframe}{\inertialframe} = \rotmat{\bodyframe}{\inertialframe}\skewMat{\angularvel{\inertialframe}{\bodyframe}{\bodyframe}} \\
\label{eq:deputy_slew}    
\dotangularvel{\inertialframe}{\bodyframe}{\bodyframe} = -\chiefInertiaInv\skewMat{\angularvel{\inertialframe}{\bodyframe}{\bodyframe}}[\chiefInertia\angularvel{\inertialframe}{\bodyframe}{\bodyframe}] + \chiefInertiaInv\tau^{\bodyframe}.
\end{gather}

The angular velocity of the $\bodyframe$ frame relative to the $\hillsframe$ frame using the property of relative angular velocity summation is 
$$\angularvel{\hillsframe}{\bodyframe}{\inertialframe} = \angularvel{\inertialframe}{\bodyframe}{\inertialframe} - \angularvel{\inertialframe}{\hillsframe}{\inertialframe}$$
with the time rate derivatives given as 
\begin{equation}
\label{eq:rel_ang_vel_inertial}
\dotangularvel{\hillsframe}{\bodyframe}{\inertialframe} = \dotangularvel{\inertialframe}{\bodyframe}{\inertialframe} - \dotangularvel{\inertialframe}{\hillsframe}{\inertialframe}.
\end{equation}
Using \eqref{eq:rotation_velocity_a} - \eqref{eq:rotation_velocity_b} and  $\angularvel{\A}{\B}{\B} = \rotmat{\A}{\B} \angularvel{\A}{\B}{\A}$ to yield the relations 
\begin{align*}
\dotangularvel{\hillsframe}{\bodyframe}{\inertialframe} &= \rotmat{\bodyframe}{\inertialframe}\skewMat{\angularvel{\inertialframe}{\bodyframe}{\bodyframe}}\angularvel{\hillsframe}{\bodyframe}{\bodyframe} + \rotmat{\bodyframe}{\inertialframe}\dotangularvel{\hillsframe}{\bodyframe}{\bodyframe} \\
\dotangularvel{\inertialframe}{\hillsframe}{\inertialframe} &= \rotmat{\hillsframe}{\inertialframe}\underbrace{\skewMat{\angularvel{\inertialframe}{\hillsframe}{\hillsframe}}\angularvel{\inertialframe}{\hillsframe}{\hillsframe}}_{=0} + \rotmat{\hillsframe}{\inertialframe}\dotangularvel{\inertialframe}{\hillsframe}{\hillsframe}  \\
\dotangularvel{\inertialframe}{\bodyframe}{\inertialframe} &= \rotmat{\bodyframe}{\inertialframe}\underbrace{\skewMat{\angularvel{\inertialframe}{\bodyframe}{\bodyframe}}\angularvel{\inertialframe}{\bodyframe}{\bodyframe}}_{=0} + \rotmat{\bodyframe}{\inertialframe}\dotangularvel{\inertialframe}{\bodyframe}{\bodyframe}
\end{align*}
substituted into a manipulation of \eqref{eq:rel_ang_vel_inertial} gives
\begin{equation}
\label{eq:relframe_quat}
\dotangularvel{\hillsframe}{\bodyframe}{\bodyframe} = \dotangularvel{\inertialframe}{\bodyframe}{\bodyframe} - \rotmat{\hillsframe}{\bodyframe}\dotangularvel{\inertialframe}{\hillsframe}{\hillsframe} - \skewMat{\angularvel{\inertialframe}{\bodyframe}{\bodyframe}}\angularvel{\hillsframe}{\bodyframe}{\bodyframe}.
\end{equation}

Let the angular velocity equations of interest be
\begin{align*}
\angularvel{\inertialframe}{\bodyframe}{\bodyframe} &:= (\omega_1 \ \omega_2 \ \omega_3)^{\top} \\
\angularvel{\hillsframe}{\bodyframe}{\bodyframe} &:= (\delta\omega_1 \ \delta\omega_2 \ \delta\omega_3)^{\top} \\
\angularvel{\inertialframe}{\hillsframe}{\bodyframe} &:= (\Omega_1 \ \Omega_2 \ \Omega_3)^{\top} \\
\end{align*}
Note that from the circular orbit assumption we have $\dotangularvel{\inertialframe}{\hillsframe}{\hillsframe} = \mathbf{0}$ and that $\angularvel{\inertialframe}{\hillsframe}{\hillsframe} = (0 \ 0 \ \meanmotion)^{\top}$ is the constant angular velocity of the Hill's frame relative to the inertial frame where
$\meanmotion$ is the constant mean motion parameter. The chief external torque vector in the $\bodyframe$ frame is $\tau^{\bodyframe} := (\tau_1 \ \tau_2 \ \tau_3)^{\top}$ and from the assumption that the chief-fixed inertia matrix is aligned with its principal axes we have $$\chiefInertia = \begin{pmatrix}
J_1 & 0 & 0 \\ 0 & J_2 & 0 \\ 0 & 0 & J_3
\end{pmatrix}.$$
Combination of \eqref{eq:deputy_slew} and \eqref{eq:relframe_quat} yields the angular velocity dynamics as
$$\dotangularvel{\hillsframe}{\bodyframe}{\bodyframe} = -\chiefInertiaInv\skewMat{\angularvel{\inertialframe}{\bodyframe}{\bodyframe}}[\chiefInertia\angularvel{\inertialframe}{\bodyframe}{\bodyframe}] + \chiefInertiaInv\tau^{\bodyframe} - \skewMat{\angularvel{\inertialframe}{\bodyframe}{\bodyframe}}\angularvel{\hillsframe}{\bodyframe}{\bodyframe}.$$
Using the relation $\angularvel{\inertialframe}{\bodyframe}{\bodyframe} = \angularvel{\hillsframe}{\bodyframe}{\bodyframe} + \angularvel{\inertialframe}{\hillsframe}{\bodyframe}$ and cross product properties the above expression becomes
\begin{align}
\label{eq:shortform_dynamics}
\begin{split}
\dotangularvel{\hillsframe}{\bodyframe}{\bodyframe} &= -\chiefInertiaInv\big(\skewMat{\angularvel{\hillsframe}{\bodyframe}{\bodyframe}}[\chiefInertia\angularvel{\hillsframe}{\bodyframe}{\bodyframe}] + \skewMat{\angularvel{\hillsframe}{\bodyframe}{\bodyframe}}[\chiefInertia\angularvel{\inertialframe}{\hillsframe}{\bodyframe}] + \\ & \qquad \qquad \qquad \qquad
\skewMat{\angularvel{\inertialframe}{\hillsframe}{\bodyframe}}[\chiefInertia\angularvel{\hillsframe}{\bodyframe}{\bodyframe}] + \skewMat{\angularvel{\inertialframe}{\hillsframe}{\bodyframe}}[\chiefInertia\angularvel{\inertialframe}{\hillsframe}{\bodyframe}]\big) + \skewMat{\angularvel{\hillsframe}{\bodyframe}{\bodyframe}}\angularvel{\inertialframe}{\hillsframe}{\bodyframe} + \chiefInertiaInv\tau^{\bodyframe}.
\end{split}
\end{align}

\subsection{Constraints}
The chief also has some constraints it must follow while performing the inspection.  Let $\tau^{\bodyframe} := [\tau_1, \ \tau_2, \ \tau_3]^{\top}$ and $\angularvel{\inertialframe}{\bodyframe}{\bodyframe} := [\omega_1, \ \omega_2, \ \omega_3]^{\top}$. Typically, the torque inputs cannot exceed some $\tau_{\max}$, and the angular velocity must be maintained under some $\omega_{\max}$. To maintain safety, the sensor cannot point in the direction of the (assumed static) sun vector $\sunvector}$ given in $\inertialframe$.
The pointing vector of the sensor is given in $\bodyframe$ as $\pointing_{\bodyframe}$.
Thus, the constraints for the chief are given in~\eqref{eq:input-constraints}-\eqref{eq:safety-constraints}.
The constraint in~\eqref{eq:safety-constraints} checks that the angle between the sun vector $\sunvector$ and $\pointing_{\inertialframe} = \rotmat{\inertialframe}{\bodyframe} \pointing_{\bodyframe}$ is at least $\alpha$.

\begin{gather}
    \norm{\tau_{k}} \leq \tau_{\max} \quad \forall k \in \{1,2,3\}
    \label{eq:input-constraints} \\
    \norm{\omega_{k}} \leq \omega_{\max} \quad \forall k \in \{1,2,3\}
    \label{eq:angvel-constraints} \\
    \sunvector^{\top}(\rotmat{\bodyframe}{\inertialframe}\pointing_{\bodyframe}) \leq \cos(\alpha)
    \label{eq:safety-constraints}
\end{gather}

% This can be expanded into
% \begin{small}
% \begin{align} 
% \label{eq:longform_dynamics}
% \begin{pmatrix}
% \delta\dot{\omega}_1 \\ \delta\dot{\omega}_2 \\ \delta\dot{\omega}_3
% \end{pmatrix}
% &= \begin{pmatrix}
% \frac{\tau_1}{J_1} + \Omega_3\delta\omega_2 - \Omega_2\delta\omega_3 + \frac{J_2 - J_3}{J_1}\delta\omega_2\delta\omega_3 + \frac{J_2 - J_3}{J_1}\Omega_2\Omega_3 + \delta\omega_3\Omega_2\frac{J_2}{J_1} - \delta\omega_2\Omega_3\frac{J_3}{J_1} + \delta\omega_2\Omega_3\frac{J_2}{J_1} - \delta\omega_3\Omega_2\frac{J_3}{J_1}\\ 
% \frac{\tau_2}{J_2} + \Omega_1\delta\omega_3 - \Omega_3\delta\omega_1 + \frac{J_3 - J_1}{J_2}\delta\omega_1\delta\omega_3 + \frac{J_3 - J_1}{J_2}\Omega_1\Omega_3 + \delta\omega_1\Omega_3\frac{J_3}{J_1} - \delta\omega_3\Omega_1\frac{J_1}{J_2} + \delta\omega_3\Omega_1\frac{J_3}{J_2} - \delta\omega_1\Omega_3\frac{J_1}{J_2}\\ 
% \frac{\tau_3}{J_3} + \Omega_2\delta\omega_1 - \Omega_1\delta\omega_2 + \frac{J_1 - J_2}{J_3}\delta\omega_1\delta\omega_2 + \frac{J_1 - J_2}{J_3}\Omega_1\Omega_2 + \delta\omega_2\Omega_1\frac{J_1}{J_3} - \delta\omega_1\Omega_2\frac{J_2}{J_3} + \delta\omega_1\Omega_2\frac{J_1}{J_3} - \delta\omega_2\Omega_1\frac{J_2}{J_3}\\ 
% \end{pmatrix}.
% \end{align}
% \end{small}


% \begin{gather}
%     \nonumber \dot{\rotmat{}{}}_{\bodyframe}^{\hillsframe} = \skewMat{\angularvel{\hillsframe}{\bodyframe}{\hillsframe}} \rotmat{\bodyframe}{\hillsframe} \\
%   \chiefInertia \dot{\angularvel{}{}{}}_{\bodyframe \inertialframe}^{\inertialframe} = -\angularvel{\bodyframe}{\inertialframe}{\inertialframe} \times \chiefInertia \angularvel{\bodyframe}{\inertialframe}{\inertialframe} + \chiefInput
% \end{gather}


% 
% 
% \kristina{There has to be a better way to talk about the resulting trajectory, come back to this.}
% Given some initial condition defined by $\rotmat{\bodyframe}{\hillsframe}(0)$ and $\angularvel{\bodyframe}{\hillsframe}{\hillsframe}(0)$,
% and torque inputs $\chiefInput(t)$, 
% the resulting trajectory of the chaser is given by $\traj:\nnreals \to \SOThree \times \reals^3$,
% which maps some time $t \geq 0$ to a rotation matrix $\rotmat{\bodyframe}{\hillsframe}(t)$ and an angular velocity $\angularvel{\bodyframe}{\hillsframe}{\hillsframe}(t)$
% such that $\traj(t) = [(\rotmat{\bodyframe}{\hillsframe}(t))^{\top} \ (\angularvel{\bodyframe}{\hillsframe}{\hillsframe}(t))^{\top}]^{\top}$.
% The trajectory $\traj(t)$ must satisfy the following:
% (i) $\traj(0) = [(\rotmat{\bodyframe}{\hillsframe}(0))^{\top} \ (\angularvel{\bodyframe}{\hillsframe}{\hillsframe}(0))^{\top}]^{\top}$, and 
% (ii) \kristina{This is where the kinematic and dynamic constraints go}.
%\begin{comment}

%\end{comment}
% 
% 
% 
\subsection{State Estimation and Tracking}
The chief is equipped with a recursive state estimator to track $m$ deputy belief states, parameterized by concatenated mean $\hat{\deputyState} := [\deputyState^{\top}_1 \ \cdots \ \deputyState^{\top}_m]^{\top}$ and covariance block matrix $\deputyUncertainty := \text{diag}\{\deputyUncertainty_1, \hdots,\deputyUncertainty_m\}$. These constructs evolve via their assumed dynamics models according to~\eqref{eq:kalman-filter}. Here, $\processNoise \in \reals^{6m \times 6m}$ is the process noise matrix and $\noiseInput \in \reals^{6m \times 6m}$ is the noise input matrix. We assume $\noiseInput = \idMat{6m}$ for simplicity.
% 
\begin{gather}
    \dot{\hat{\deputyState}} = (\idMat{m} \otimes \deputyStateMat) \hat{\deputyState} \nonumber \\
    \dot{\deputyUncertainty} = (\idMat{m} \otimes \deputyStateMat) \deputyUncertainty (\idMat{m} \otimes \deputyStateMat)^{\top} + \noiseInput \processNoise \noiseInput^{\top}
    \label{eq:kalman-filter}
\end{gather}
% 
where $\otimes$ is the Kronecker product.
The chief is equipped with a sensor that can observe the states of deputies that are within the sensing field-of-view (FOV).
The sensor has a conical FOV defined by the angle of view $\alpha$, the pointing direction in the body frame $\pointing_{\bodyframe}$, and is fixed on the chief frame with defined orientation $\rotmat{\bodyframe}{\inertialframe}$.
Thus, the measurement model is given by $\obsState = \obsMat(\deputyState, \rotmat{\bodyframe}{\inertialframe}}) \deputyState$
where $\obsState$ gives the observed states of the deputies 
and $\deputyState = [\deputyState^{\top}_1 \ \cdots \ \deputyState^{\top}_m]^{\top}$ are the actual states of all the deputies.
The observation matrix $\obsMat$ is defined as the block matrix in~\eqref{eq:obsMat},
where each $\obsMat_i(\deputyState_i,\rotmat{\bodyframe}{\inertialframe})$, $i \in [1, m]$ is the observation matrix for deputy $i$ given in~\eqref{eq:deputy_obs}.

\begin{equation}
    \obsMat(\deputyState, \rotmat{\bodyframe}{\inertialframe}) = \begin{bmatrix}
    \obsMat_1(\deputyState_1, \rotmat{\bodyframe}{\inertialframe}) & \emptyMat{6}{6} & \cdots & \emptyMat{6}{6}\\
    \emptyMat{6}{6} & \obsMat_2(\deputyState_2, \rotmat{\bodyframe}{\inertialframe}) & \cdots & \emptyMat{6}{6}\\
    \vdots & \vdots & \ddots & \vdots\\
    \emptyMat{6}{6} & \emptyMat{6}{6} & \cdots & \obsMat_m(\deputyState_m, \rotmat{\bodyframe}{\inertialframe})
        %\obsMat_1(\deputyState_1, \rotmat{\bodyframe}{\inertialframe}) & \zeroMat{6}{6} & \cdots & \zeroMat{6}{6} \\
        %\zeroMat{6}{6} & \obsMat_2(\deputyState_2, \rotmat{\bodyframe}{\inertialframe}) & \cdots & \zeroMat{6}{6} \\
        %\vdots & \vdots & \ddots & \vdots \\
        %\zeroMat{6}{6} & \zeroMat{6}{6} & \cdots & \obsMat_n(\deputyState_n, \rotmat{\bodyframe}{\inertialframe}) \\
    \end{bmatrix}
    \label{eq:obsMat}
\end{equation}

\begin{equation}
    \obsMat_i(\deputyState_i, \rotmat{\bodyframe}{\inertialframe}) = \begin{cases}
        \idMat{6} & \cos^{-1}(\rotmat{\bodyframe}{\inertialframe} \pointing_{\bodyframe} \cdot \deputyState_i) \leq \alpha \\
        \emptyMat{6}{6} & \textrm{else}
    \end{cases}, \quad i = 1, 2, \dots, m
    \label{eq:deputy_obs}
\end{equation}

It should be noted here that $\emptyMat{6}{6}$ is an overloaded operator.
In the case that $\obsMat_i(\deputyState_i, \rotmat{\bodyframe}{\inertialframe}) = \idMat{6}$, $\emptyMat{6}{6}$ takes on the value of $\zeroMat{6}{6}$, and in the case when $\obsMat_i(\deputyState_i, \rotmat{\bodyframe}{\inertialframe}) = \emptyMat{6}{6}$, $\emptyMat{6}{6}$ takes on the meaning of an empty matrix. 
This is done to ensure the proper dimensionality of the system is maintained during observations, and it is clear that the chief cannot observe any more states than is currently within its FOV.

Whenever the chief makes an observation of a deputy state at a time instant $t_k$, the measurement data is incorporated by the on-board estimator to impulsively update the belief state, i.e. 
$$(\hat{\deputyState}^{-}(t_k), \deputyUncertainty^{-}(t_k)) \rightarrow (\hat{\deputyState}^{+}(t_k), \deputyUncertainty^{+}(t_k)).$$
As a result, the size of the covariance matrices of observed deputies will necessarily decrease $\det[\deputyUncertainty^{+}_i] \leq \det[\deputyUncertainty^{-}_i]$ and the updated belief state will be recursively supplied to the propagator until the next available measurement update. However, because the sensor has a limited FOV, it may not be possible for the chief to observe every deputy at once. Therefore, the chief must maneuver to view each deputy to maintain a level of certainty in the state estimate.
%estimated states of the deputies $\hat{\deputyState}$ is updated by replacing the values in $\hat{\deputyState}$ with the corresponding non-zero entries in $\obsState$,
%and the corresponding $\deputyUncertainty_i$'s are \kristina{reset?}.
%\kristina{Discuss timing of the algorithm in this paragraph}
\subsection{Constraints}
The chief also has some constraints it must follow while performing the inspection.  Let $\tau^{\bodyframe} := [\tau_1, \ \tau_2, \ \tau_3]^{\top}$ and $\angularvel{\inertialframe}{\bodyframe}{\bodyframe} := [\omega_1, \ \omega_2, \ \omega_3]^{\top}$. Typically, the torque inputs cannot exceed some $\tau_{\max}$, and the angular velocity must be maintained under some $\omega_{\max}$. To maintain safety, the sensor cannot point in the direction of the (assumed static) sun vector $\sunvector}$ given in $\inertialframe$.
The pointing vector of the sensor is given in $\bodyframe$ as $\pointing_{\bodyframe}$.
Thus, the constraints for the chief are given in~\eqref{eq:input-constraints}-\eqref{eq:safety-constraints}.
The constraint in~\eqref{eq:safety-constraints} checks that the angle between the sun vector $\sunvector$ and $\pointing_{\inertialframe} = \rotmat{\inertialframe}{\bodyframe} \pointing_{\bodyframe}$ is at least $\alpha$.

\begin{gather}
    \norm{\tau_{k}} \leq \tau_{\max} \quad \forall k \in \{1,2,3\}
    \label{eq:input-constraints} \\
    \norm{\omega_{k}} \leq \omega_{\max} \quad \forall k \in \{1,2,3\}
    \label{eq:angvel-constraints} \\
    \sunvector^{\top}(\rotmat{\bodyframe}{\inertialframe}\pointing_{\bodyframe}) \leq \cos(\alpha)
    \label{eq:safety-constraints}
\end{gather}

\subsection{Optimal Control Problem Statement}
In summary,  the local catalog maintenance problem is then given by the following optimal control problem.
Given a chief satellite in a circular orbit about the earth defined by $\meanmotion$, and $n$ deputy satellites, each in an closed elliptical NMT, find some input $\chiefInput(t)$
that optimizes
\begin{equation}\label{eq:ocp}
        J &= f(\hat{\deputyState}, \deputyUncertainty, \chiefInput)\\
\end{equation}
subject to,
\begin{equation*}
\begin{aligned}
\textrm{Deputy Translational Dynamics}&
\begin{cases}
\dot{\deputyState} &= (\idMat{m} \otimes \deputyStateMat)\deputyState\\
\end{cases} \\
\textrm{Chief Rotational Dynamics}&
\begin{cases}
\dotrotmat{\bodyframe}{\inertialframe} &= \rotmat{\bodyframe}{\inertialframe}\skewMat{\angularvel{\inertialframe}{\bodyframe}{\bodyframe}}\\
\dotangularvel{\inertialframe}{\bodyframe}{\bodyframe} &= -\chiefInertiaInv\skewMat{\angularvel{\inertialframe}{\bodyframe}{\bodyframe}}[\chiefInertia\angularvel{\inertialframe}{\bodyframe}{\bodyframe}] + \chiefInertiaInv\tau^{\bodyframe}
\end{cases}\\
\textrm{Chief Rotational Constraints}&
\begin{cases}
  \norm{\tau_{k}} &\leq \tau_{\max} \quad \forall k \in \{1,2,3\} \\
    \norm{\omega_{k}} &\leq \omega_{\max} \quad \forall k \in \{1,2,3\}\\
    \sunvector^{\top}(\rotmat{\bodyframe}{\inertialframe}\pointing_{\bodyframe}) &\leq \cos(\alpha)
\end{cases}\\
\textrm{Belief State Propagation}&
\begin{cases}
  \dot{\hat{\deputyState}} &= (\idMat{m} \otimes \deputyStateMat) \hat{\deputyState} \nonumber \\
    \dot{\deputyUncertainty} &= (\idMat{m} \otimes \deputyStateMat) \deputyUncertainty (\idMat{m} \otimes \deputyStateMat)^{\top} + \noiseInput \processNoise \noiseInput^{\top}
\end{cases}\\
\textrm{Chief Observation}&
\begin{cases}
\obsState &= \obsMat(\deputyState, \rotmat{\bodyframe}{\inertialframe}}) \deputyState
\end{cases}
\end{aligned}
\end{equation*}

Furthermore, it is assumed that the constraints are satisfied for all $t \geq 0$, and the cost function $J$ is continuous, continually differentiable, and non-negative.
Implicitly, the posed optimal control problem consists of two parts: which deputy to view, and how to maneuver to view it?
With this in mind, the following section describes how each of these subproblems is addressed.
%\kristina{constraints are satisfied for all $t \geq 0$},
%and
%\kristina{covariance matrix is bounded}.

%\kristina{The cost function, etc. should be discussed in the methodology section.}


\begin{comment}
% \section{Preliminaries}
% \subsection{Relative Orbital Mechanics}
% \subsubsection{Clohessy-Wiltshire-Hill Equations}
% The Clohessy-Wiltshire-Hill (CWH) equations \cite{clohessy1960terminal} have become fundamental in describing the relative orbital dynamics of multi-satellite configurations operating within close proximity of a circular orbit.
% By leveraging Hill's Frame \cite{hill1878researches}, the CWH equations provide a linear approximation of the dynamics of such systems and allow for associated linear analysis techniques to be applied.
% The full CWH equations of motion are shown in Equation \eqref{eq: cw_equations}
% \begin{equation}\label{eq: cw_equations}
%     \begin{split}
%         \dot{v}_{x} &= 2nv_{y}+3n^2r_{x}+u_{x} \\
%         \dot{v}_{y} &= -2nv_{x}+u_{y}\\
%         \dot{v}_{z} &= -n^2r_{z} + u_{z}
%     \end{split}
% \end{equation}
% Where $n$ is the mean motion of Hill's Frame around the earth. 
% Alternatively, these same equations may be placed in the form of a standard linear system, $\dot{\textbf{x}}=\textbf{A}\textbf{x}+\textbf{B}\textbf{u}$, $\textbf{y}=\textbf{C}\textbf{x}$ where the state matrix $\textbf{A}$, control matrix $\textbf{B}$ are defined in Equation \eqref{eq: state and control}.
% The measurement matrix $\textbf{C}$ is discussed in more detail in Section \ref{sec: system_consideration}
%  \begin{equation} \label{eq: state and control}
%  \textbf{A} =
% \begin{bmatrix} 
% 0 & 0 & 0 & 1 & 0 & 0\\
% 0 & 0 & 0 & 0 & 1 & 0\\
% 0 & 0 & 0 & 0 & 0 & 1\\
% 3n^2& 0 & 0 & 0 & 2n & 0\\
% 0 & 0 & 0 & -2n & 0 & 0\\
% 0 & 0 & -n^2 & 0 & 0 & 0\\
% \end{bmatrix} , 
% \quad 
% \textbf{B} = 
% \begin{bmatrix}
% 0 & 0 & 0\\
% 0 & 0 & 0\\
% 0 & 0 & 0\\
% 1 & 0 & 0\\
% 0 & 1& 0\\
% 0 & 0 & 1\\
% \end{bmatrix} ,
% \quad
% \end{equation}

% For multi-satellite systems, the above linear description may be expanded as $\dot{\textbf{x}} = \bar{\textbf{A}}\textbf{x}+\bar{\textbf{B}}\textbf{u}$ and $\textbf{y} = \bar{\textbf{C}}\textbf{x}$, where $\bar{\textbf{A}} = (I_{n}\otimes \textbf{A})$, $\bar{\textbf{B}} = (I_{n}\otimes \textbf{B})$, and $\bar{\textbf{C}} = (I_{p}\otimes \textbf{C})$
% Where $\otimes$ denotes the Kronecker product, $I_{n}$ is the $n$-dimensional identity matrix, and now, the state vector $\textbf{x}$ is the augmentation of each of the individual satellite state vectors, $\textbf{x}=[\textbf{x}^T_{1},\ \dots,\ \textbf{x}_{n}^{T}]^{T}$.

% \subsubsection{Natural Motion Trajectories}\label{sec: nmt}

% A class of periodic solutions exist to the CWH equations for when $\textbf{u}=0$.
% This particular class of solutions are often referred to as Natural Motion Trajectories (NMTs) or Passive Relative Orbits (PROs) and have been extensively used for a wide variety of relative orbital motion problems \cite{shibata2007orbital}, \cite{mote2021natural}, \cite{frey2017incorporating}, \cite{hobbs2020taxonomy}, \cite{soderlund2022autonomous}.
% First pointed out in \cite{kim2007mission} and expanded upon in \cite{frey2017constrained}, the NMTs themselves can take the form of stationary points, lines, ellipses, or spirals depending on the inital conditions of the satellite.
% All of the forms must first meet the initial condition $v_{y} = -2nr_{x}$.
% Additional specific initial conditions for each NMT form is specified below:
% \begin{enumerate}
%     \item \textit{Stationary Point}: $r_{x}=r_{z} = v_{x} = v_{z} = 0$
%     \item \textit{Line Segment}:  $r_{x} = v_{x} = 0$, $r_{z} = c\text{sin}(\psi)$, and $v_{z} = n c \text{cos}(\psi)$
%     \item \textit{Ellipse}:  $v_{x} = \frac{n}{2}r_{y}$
% \end{enumerate}
% Where $c$ is the amplitude of the length segment in the $\hat{z}$ direction, and $\psi$ is the initial angle between the agent and the $x-y$ plane.

\section{Problem Formulation}
\label{sec: problem_formulation}

\paragraph{Preliminaries}
\kristina{The mathematical preliminaries should go here}

Consider the reverse satellite inspection problem, where a chief satellite is tasked with inspecting and monitoring several deputy satellites.
Here, the chief can rotate about the origin of a reference frame affixed to its center of mass (Hill's frame).
As the chief rotates, it can take measurements of the states of deputies that enter its field of view (FOV).
The uncertainty of the state of a deputy increases as the time since its last inspection increases.
The reverse satellite inspection problem is then to find a trajectory for the chief to take such that the uncertainty never grows too large.
In this section, we will formalize the reverse satellite inspection problem.

\subsection{Deputy agents}
Consider the problem with $m$ deputy agents.
Let the state of each deputy $i \in [1, N]$ be given by $\deputyState_{i} \in \deputyStateSpace_{i} \subset \reals^{6}$,
where $\deputyState_i = [r_{i,x} \ r_{i,y} \ r_{i,z} \ v_{i,x} \ v_{i,y} \ v_{i,z}]^{\top}$.
The state of each deputy evolves according to $\dot{\deputyState}_i = \deputyStateMat \deputyState_i$,
where $\deputyStateMat$ is given in~\eqref{eq: state and control}, using the Clohessy-Wiltshire-Hill equations.
% 
% \paragraph{Clohessy-Wiltshire-Hill Equations}
The Clohessy-Wiltshire-Hill (CWH) equations \cite{clohessy1960terminal} have become fundamental in describing the relative orbital dynamics of multi-satellite configurations operating within close proximity of a circular orbit.
By leveraging Hill's Frame \cite{hill1878researches}, the CWH equations provide a linear approximation of the dynamics of such systems and allow for associated linear analysis techniques to be applied.
The full CWH equations of motion are shown in~\eqref{eq: cw_equations}.
% \begin{equation}\label{eq: cw_equations}
%     \begin{split}
%         \dot{v}_{x} &= 2nv_{y}+3n^2r_{x}+u_{x} \\
%         \dot{v}_{y} &= -2nv_{x}+u_{y}\\
%         \dot{v}_{z} &= -n^2r_{z} + u_{z}
%     \end{split}
% \end{equation}
\begin{gather}
    \dot{v}_{x} = 2nv_{y}+3n^2r_{x} \nonumber \\
    \dot{v}_{y} = -2nv_{x} \nonumber \\
    \dot{v}_{z} = -n^2r_{z} \label{eq: cw_equations}
\end{gather}

Where $n$ is the mean motion of Hill's Frame around the earth. 
Typically, $n=0.0012$ for low earth orbit.
The state matrix is then given in~\eqref{eq: state and control}.
% Alternatively, these same equations may be placed in the form of a standard linear system, $\dot{\textbf{x}}=\textbf{A}\textbf{x}+\textbf{B}\textbf{u}$, $\textbf{y}=\textbf{C}\textbf{x}$ where the state matrix $\textbf{A}$, control matrix $\textbf{B}$ are defined in Equation \eqref{eq: state and control}.
% The measurement matrix $\textbf{C}$ is discussed in more detail in Section \ref{sec: system_consideration}
%  \begin{equation} \label{eq: state and control}
%  \textbf{A} =
% \begin{bmatrix} 
% 0 & 0 & 0 & 1 & 0 & 0\\
% 0 & 0 & 0 & 0 & 1 & 0\\
% 0 & 0 & 0 & 0 & 0 & 1\\
% 3n^2& 0 & 0 & 0 & 2n & 0\\
% 0 & 0 & 0 & -2n & 0 & 0\\
% 0 & 0 & -n^2 & 0 & 0 & 0\\
% \end{bmatrix} , 
% \quad 
% \textbf{B} = 
% \begin{bmatrix}
% 0 & 0 & 0\\
% 0 & 0 & 0\\
% 0 & 0 & 0\\
% 1 & 0 & 0\\
% 0 & 1& 0\\
% 0 & 0 & 1\\
% \end{bmatrix} ,
% \quad
% \end{equation}
\begin{equation} 
\deputyStateMat =
\begin{bmatrix} 
0 & 0 & 0 & 1 & 0 & 0\\
0 & 0 & 0 & 0 & 1 & 0\\
0 & 0 & 0 & 0 & 0 & 1\\
3n^2& 0 & 0 & 0 & 2n & 0\\
0 & 0 & 0 & -2n & 0 & 0\\
0 & 0 & -n^2 & 0 & 0 & 0\\
\end{bmatrix}
\label{eq: state and control}
\end{equation}

For multi-satellite systems, the above linear description may be expanded as $\dot{\deputyState} = \bar{\deputyStateMat}\deputyState$,
% +\bar{\textbf{B}}\textbf{u}$ and $\textbf{y} = \bar{\textbf{C}}\textbf{x}$
where $\bar{\deputyStateMat} = (\idMat_{N}\otimes \deputyStateMat)$,
% $\bar{\textbf{B}} = (I_{N}\otimes \textbf{B})$, and $\bar{\textbf{C}} = (I_{p}\otimes \textbf{C})S
where $\otimes$ denotes the Kronecker product, $\idMat_{N}$ is the $N$-dimensional identity matrix, 
and the augmented state vector
% and now, the state vector $\textbf{x}$ is the augmentation of each of the individual satellite state vectors,
$\deputyStateMat=[\deputyState_1^{\top},\ \dots, \ \deputyState_{N}^{\top}]^{\top}$.

\subsubsection{Natural Motion Trajectories.}\label{sec: nmt}

A class of periodic solutions exist to the CWH equations for when $\textbf{u}=0$.
This particular class of solutions are often referred to as Natural Motion Trajectories (NMTs) or Passive Relative Orbits (PROs) and have been extensively used for a wide variety of relative orbital motion problems \cite{shibata2007orbital, mote2021natural, frey2017incorporating, hobbs2020taxonomy, soderlund2022autonomous}.
First pointed out in \cite{kim2007mission} and expanded upon in \cite{frey2017constrained}, the NMTs themselves can take the form of stationary points, lines, ellipses, or spirals depending on the inital conditions of the satellite.
For any satellite $i \in [1, N]$, any form of NMT must meet the initial condition
% All of the forms must first meet the initial condition 
$v_{i,y} = -2nr_{x}$.
Additional 
% specific 
initial conditions for each NMT form are specified below:
\begin{enumerate}
    \item \textit{Stationary Point}: $r_{i,x}=r_{i,z} = v_{i,x} = v_{i,z} = 0$
    \item \textit{Line Segment}:  $r_{i,x} = v_{i,x} = 0$, $r_{i,z} = c \sin(\psi)$, and $v_{i,z} = n c \cos(\psi)$
    \item \textit{Ellipse}:  $v_{i,x} = \frac{n}{2}r_{i,y}$
\end{enumerate}
Where $c$ is the amplitude of the length segment in the $\hat{z}$ direction, and $\psi$ is the initial angle between the agent and the $x-y$ plane.

\subsection{Chief agent}
The chief agent is strategically placed at the origin of the Global Frame and only capable of rotational motion.
The rotation matrix of the chief is given by $\chiefState \in \SOThree$,
and the angular velocities $\chiefVels \in \reals^3$ where $\chiefVels = [\chiefVel_1 \ \chiefVel_2 \ \chiefVel_3]^{\top}$.
The state of the chaser evolves according to~\eqref{eq: chiefAttitude.}.
Here, $\chiefInput$ is the torque control input, and $\skewMat{\chiefVels}$ is the skew-symmetric matrix of angular velocities given by~\eqref{eq: skewMat}

\begin{gather}
    \dot{\chiefState} = \chiefState \skewMat{\chiefVels} \nonumber \\
    \chiefInertia \dot{\chiefVels} = -\chiefVels \times \chiefInertia + \chiefInput
    \label{eq: chiefAttitude.}
\end{gather}    
% 
\begin{equation}
    \skewMat{\chiefVels} = \begin{bmatrix}
        0 & -\chiefVel_3 & \chiefVel_2 \\
        \chiefVel_3 & 0 & -\chiefVel_1 \\
        -\chiefVel_2 & \chiefVel_1 & 0
    \end{bmatrix} 
    \label{eq: skewMat}
\end{equation}

\subsection{Measurement model}

The chief is also equipped with a sensor capable of measuring the position of each agent as long as the agent is within the sensor's field-of-view (FOV) defined by the angles $\alpha$. Mathematically, a measurement is taken only when $\textbf{x}\in \boldsymbol{\mathcal{X}}_{fov} \subset \boldsymbol{\mathcal{X}}$ where $\boldsymbol{\mathcal{X}}_{fov}$ is the subset of all admissible $\textbf{x}$ that exist within the sensor's FOV at a given time instant.
The measurement function is given by the linear system
\begin{equation}
    \textbf{y} = \textbf{C}(\textbf{x}, \textbf{R})\textbf{x}
\end{equation}
where $\textbf{C}(\textbf{x}, \textbf{R}) \in {\mathbb R}^{6n\times 6n}$ is an implicit time-varying measurement matrix. 
Explicitly, this measurement matrix is dependent on the position of Agents $1,\dots,n$ and the orientation of Agent 0.
$\textbf{C(x, R)}$ is constructed as a block-diagonal matrix with the identity matrix, $\textbf{I}$, placed in the indices within the sensor's FOV.
\begin{equation*}
    \textbf{C(x,\ R)} = blckdiag([\textbf{C}_{i}])\ \forall i=1,\dots,n
\end{equation*}
where,
\begin{equation*}
    \textbf{C}_{i}=\Big\{\begin{array}{cc}
        \textbf{I}, & \textbf{x} \in \boldsymbol{\mathcal{X}}_{fov} \\
      \boldsymbol{0},  & \textbf{x} \notin \boldsymbol{\mathcal{X}}_{fov}
    \end{array}
\end{equation*}
and the condition for the state vector existing within the sensor's FOV is defined as
\begin{equation}
\cos^{-1}(\textbf{n}\cdot\textbf{x})\leq \alpha \Rightarrow \textbf{x}\in\boldsymbol{\mathcal{X}}_{fov}
\end{equation}
with $\textbf{n}$ being the pointing direction of the sensor.

\subsection{Kalman Filter}

Furthermore, it is assumed the chief is equipped with a Kalman Filter to track the states and uncertainties of the Agents $1,\dots,n$.

\begin{equation}
\begin{split}
    \dot{\hat{\textbf{\deputyState}}} &= \deputyStateMat \hat{\textbf{x}}+\textbf{Bu} \\
    \dot{\textbf{P}} &= \textbf{APA}^T + \textbf{GQG}^T 
    \end{split}
\end{equation}
where $\hat{\textbf{x}}$ is the state estimate, $\textbf{P}$ is the state covariance matrix, $\textbf{Q}$ is the process noise matrix, and $\textbf{G}$ is the noise input matrix.
For simplicity, $\textbf{G}=\textbf{I}$.
It is also assumed that Agent 0 is perfectly aware of its own orientation $\textbf{R}$.
The goal is now for Agent 0 to autonomously track and monitor Agents $1,\dots,n$ by minimizing the state uncertainty of every agent in the system.

\subsection{Inspection and uncertainties}
Let us consider the state of the inspection to be $\inspectState = [\hat{\deputyState}, \deputyUncertainty]^{\top}$,
where 
$\deputyState = [\deputyState_1 \ \cdots 
\ \deputyState_N]^{\top}$
is the state of the $N$ deputies,
$\hat{\deputyState}$ is the chief's estimate of the deputies states, and 
$\deputyUncertainty = [\deputyUncertainty_1 \ \cdots \ \deputyUncertainty_N]$ is the uncertainty in each of the deputies states.
The state of each deputy evolves according to some linear time invariant (LTI) system $\dot{\deputyState} = A\deputyState$,
thus the estimate of the deputie's states evolves according to
$\dot{\hat{\deputyState}} = A\hat{\deputyState}$.
Furthermore, the uncertainty $\deputyUncertainty_i$ associated with each deputy $i \in [0, N]$ grows monotonically according to 
\begin{equation}
    \dot{\deputyUncertainty}_{i} = A\deputyUncertainty_{i} A^T
\end{equation}
Then, when the chief makes no observations, the state of the inspection evolves according to the following equation:
\begin{equation}
    \dot{\inspectState} = \begin{bmatrix}
    \dot{\hat{\deputyState}} \\ \dot{\deputyUncertainty}
    \end{bmatrix} = \begin{bmatrix}
    (\idMat_N \otimes A) \hat{\deputyState} \\
    (\idMat_N \otimes A) \deputyUncertainty (\idMat_N \otimes A^{\top})
    \end{bmatrix}.
\end{equation}

The satellite inspection problem is then 


% \kristina{
% In the reverse satellite inspection problem, the chief must periodically make observations of the deputies.
% When a deputy is observed, the uncertainty associated with that deputy is reduced.
% Thus, the state of the inspection evolves according to the following equation:
% \begin{equation}
%     \dot{\inspectState} = \begin{bmatrix}
%     \dot{\hat{\deputyState}} \\ \dot{\deputyUncertainty}
%     \end{bmatrix} = \begin{bmatrix}
%     (I \otimes A) \hat{\deputyState} \\
%     (I \otimes A) \deputyUncertainty (I \otimes A^{\top})
%     \end{bmatrix} + \begin{bmatrix}
%     \obsCorrection \\ \uncertaintyCorrection
%     \end{bmatrix}
% \end{equation}
% where $\obsCorrection = [\obsCorrection_1 \ \cdots \ \obsCorrection_N]^{\top}$ is the \textcolor{red}{observation correction factor?} and $\uncertaintyCorrection = [\uncertaintyCorrection_1 \ \cdots \ \uncertaintyCorrection_N]^{\top}$ is the \textcolor{red}{uncertainty correction factor?} which updates the state and uncertainty of a deputy each time an observation is made.
% }

% \kristina{
% The chief can make an observation by pointing a sensor at a deputy.
% The chief can move the sensor by rotating about the center of Hill's frame.
% The dynamics of the chief are given by the following:
% \begin{gather}
%     \dot{\textbf{R}} = \textbf{R}\boldsymbol{\omega}^{\times} \\
%     \dot{\boldsymbol{\omega}} = \boldsymbol{\tau}.
% \end{gather}
% The field of view of the sensor is given by the following:
% \begin{equation}
% \cos^{-1}(\textbf{n}\cdot\textbf{x})\leq \alpha \Rightarrow \textbf{x}\in\boldsymbol{\mathcal{X}}_{fov}
% \end{equation}
% with $\textbf{n}$ being the pointing direction of the sensor.
% }

% \kristina{
% In the reverse satellite inspection problem, the chief must make observations that keep the uncertainty bounded.
% Additionally, the sensors on the chief must remain safe with respect to some sun vectors.
% Let the set of states at any time $t$ that keeps the sensors on the chief safe be given by $\workspace$ $(t)$.
% Then, we want to find $\tau$ such that
% $\Sigma(t) \leq \varepsilon$ for all $t$
% and 
% $\textbf{R} \in \workspace$ for all $t$.
% }

\subsection{Constraints}

- Kinematic and Dynamic Constraints

-- Must follow physics, Decide on attitude parameterization set

- Boundary Constraints

-- Control Torque Bounds, Angular Velocity Bounds, Uncertainty Bounds

- Pointing Exclusion Zones

-- Don't point at sun

\subsection{Problem statement}

In general, this case may be classified as a Perception-Aware Chance-Constrained Optimal Control Problem. 
\cite{bonzanini2021perception, bonzanini2021stability}
\kristina{Probelm statement goes here}








% Let us consider the state of the inspection to be $\inspectState = [\hat{\deputyState}, \deputyUncertainty]^{\top}$,
% where 
% $\deputyState = [\deputyState_1 \ \cdots 
% \ \deputyState_N]^{\top}$
% is the state of the $N$ deputies,
% $\hat{\deputyState}$ is the chief's estimate of the deputies states, and 
% $\deputyUncertainty = [\deputyUncertainty_1 \ \cdots \ \deputyUncertainty_N]$ is the uncertainty in each of the deputies states.
% The state of each deputy evolves according to some linear time invariant (LTI) system $\dot{\deputyState} = A\deputyState$,
% thus the estimate of the deputie's states evolves according to
% $\dot{\hat{\deputyState}} = A\hat{\deputyState}$.
% Furthermore, the uncertainty $\deputyUncertainty_i$ associated with each deputy $i \in [0, N]$ grows monotonically according to 
% \begin{equation}
%     \dot{\deputyUncertainty}_{i} = A\deputyUncertainty_{i} A^T
% \end{equation}
% Then, when the chief makes no observations, the state of the inspection evolves according to the following equation:
% \begin{equation}
%     \dot{\inspectState} = \begin{bmatrix}
%     \dot{\hat{\deputyState}} \\ \dot{\deputyUncertainty}
%     \end{bmatrix} = \begin{bmatrix}
%     (I \otimes A) \hat{\deputyState} \\
%     (I \otimes A) \deputyUncertainty (I \otimes A^{\top})
%     \end{bmatrix}.
% \end{equation}


% \kristina{
% In the reverse satellite inspection problem, the chief must periodically make observations of the deputies.
% When a deputy is observed, the uncertainty associated with that deputy is reduced.
% Thus, the state of the inspection evolves according to the following equation:
% \begin{equation}
%     \dot{\inspectState} = \begin{bmatrix}
%     \dot{\hat{\deputyState}} \\ \dot{\deputyUncertainty}
%     \end{bmatrix} = \begin{bmatrix}
%     (I \otimes A) \hat{\deputyState} \\
%     (I \otimes A) \deputyUncertainty (I \otimes A^{\top})
%     \end{bmatrix} + \begin{bmatrix}
%     \obsCorrection \\ \uncertaintyCorrection
%     \end{bmatrix}
% \end{equation}
% where $\obsCorrection = [\obsCorrection_1 \ \cdots \ \obsCorrection_N]^{\top}$ is the \textcolor{red}{observation correction factor?} and $\uncertaintyCorrection = [\uncertaintyCorrection_1 \ \cdots \ \uncertaintyCorrection_N]^{\top}$ is the \textcolor{red}{uncertainty correction factor?} which updates the state and uncertainty of a deputy each time an observation is made.
% }

% \kristina{
% The chief can make an observation by pointing a sensor at a deputy.
% The chief can move the sensor by rotating about the center of Hill's frame.
% The dynamics of the chief are given by the following:
% \begin{gather}
%     \dot{\textbf{R}} = \textbf{R}\boldsymbol{\omega}^{\times} \\
%     \dot{\boldsymbol{\omega}} = \boldsymbol{\tau}.
% \end{gather}
% The field of view of the sensor is given by the following:
% \begin{equation}
% \cos^{-1}(\textbf{n}\cdot\textbf{x})\leq \alpha \Rightarrow \textbf{x}\in\boldsymbol{\mathcal{X}}_{fov}
% \end{equation}
% with $\textbf{n}$ being the pointing direction of the sensor.
% }

% \kristina{
% In the reverse satellite inspection problem, the chief must make observations that keep the uncertainty bounded.
% Additionally, the sensors on the chief must remain safe with respect to some sun vectors.
% Let the set of states at any time $t$ that keeps the sensors on the chief safe be given by $\workspace$ $(t)$.
% Then, we want to find $\tau$ such that
% $\Sigma(t) \leq \varepsilon$ for all $t$
% and 
% $\textbf{R} \in \workspace$ for all $t$.
% }

% \textcolor{red}{We are missing a few connections between the inspection state and chief state, but this should be the general gist of the problem.}

% \subsection{System Dynamics}
% Suppose Agent 0 is tasked with measuring and tracking the positions of Agents $1,\dots,n$.
% Each of Agents $1,\dots, n$ evolve in the Global Frame as a Linear-Time Invariant (LTI) system
% \begin{equation}
%     \dot{\textbf{x}} = \textbf{A}\textbf{x} + \textbf{B}\textbf{u}
% \end{equation}
% where $\textbf{A}\in\mathbb{R}^{6n\times 6n}$, $\textbf{B}\in \mathbb{R}^{6n\times p}$ with $p$ being the number of control inputs, $\textbf{x} \in \boldsymbol{\mathcal{X}}$ with $\boldsymbol{\mathcal{X}}$ being the set of all admissible states, and $\textbf{u} \in \boldsymbol{\mathcal{U}}$ with $\boldsymbol{\mathcal{U}}$ being the set of all admissible control inputs.
% Agent 0 is strategically placed at the origin of the Global Frame and only capable of rotational motion

% \begin{equation}
%     \dot{\textbf{R}} = \textbf{R}\boldsymbol{\omega}^{\times}
% \end{equation}
% \begin{equation}
%     J\dot{\boldsymbol{\omega}} = -\boldsymbol{\omega}\times \boldsymbol{J\boldsymbol{\omega}}+(\boldsymbol{\tau}+\boldsymbol{u})
% \end{equation}
% where $\textbf{R}\in SO(3)$ is the rotation matrix, $\boldsymbol{\tau}$ is the torque control input, and $\boldsymbol{\omega}$ is the skew-symmetric matrix of angular velocities.
% \begin{equation*}
%     \boldsymbol{\omega}^{\times} = 
%     \begin{bmatrix}
%     0 & -\omega_3 & \omega_2 \\
%     \omega_3 & 0 & -\omega_1 \\
%     -\omega_2 & \omega_1 & 0
%     \end{bmatrix}
% \end{equation*}

% \subsection{Measurement Model}
% Agent 0 is also equipped with a sensor capable of measuring the position of each agent as long as the agent is within the sensor's field-of-view (FOV) defined by the angles $\alpha$. Mathematically, a measurement is taken only when $\textbf{x}\in \boldsymbol{\mathcal{X}}_{fov} \subset \boldsymbol{\mathcal{X}}$ where $\boldsymbol{\mathcal{X}}_{fov}$ is the subset of all admissible $\textbf{x}$ that exist within the sensor's FOV at a given time instant.
% The measurement function is given by the linear system
% \begin{equation}
%     \textbf{y} = \textbf{C}(\textbf{x}, \textbf{R})\textbf{x}
% \end{equation}
% where $\textbf{C}(\textbf{x}, \textbf{R}) \in {\mathbb R}^{6n\times 6n}$ is an implicit time-varying measurement matrix. 
% Explicitly, this measurement matrix is dependent on the position of Agents $1,\dots,n$ and the orientation of Agent 0.
% $\textbf{C(x, R)}$ is constructed as a block-diagonal matrix with the identity matrix, $\textbf{I}$, placed in the indices within the sensor's FOV.
% \begin{equation*}
%     \textbf{C(x,\ R)} = blckdiag([\textbf{C}_{i}])\ \forall i=1,\dots,n
% \end{equation*}
% where,
% \begin{equation*}
%     \textbf{C}_{i}=\Big\{\begin{array}{cc}
%         \textbf{I}, & \textbf{x} \in \boldsymbol{\mathcal{X}}_{fov} \\
%       \boldsymbol{0},  & \textbf{x} \notin \boldsymbol{\mathcal{X}}_{fov}
%     \end{array}
% \end{equation*}
% and the condition for the state vector existing within the sensor's FOV is defined as
% \begin{equation}
% \cos^{-1}(\textbf{n}\cdot\textbf{x})\leq \alpha \Rightarrow \textbf{x}\in\boldsymbol{\mathcal{X}}_{fov}
% \end{equation}
% with $\textbf{n}$ being the pointing direction of the sensor.

% Furthermore, it is assumed Agent 0 is equipped with a Kalman Filter to track the states and uncertainties of the Agents $1,\dots,n$.

% \begin{equation}
% \begin{split}
%     \dot{\hat{\textbf{x}}} &= \textbf{A}\hat{\textbf{x}}+\textbf{Bu} \\
%     \dot{\textbf{P}} &= \textbf{APA}^T + \textbf{GQG}^T 
%     \end{split}
% \end{equation}
% where $\hat{\textbf{x}}$ is the state estimate, $\textbf{P}$ is the state covariance matrix, $\textbf{Q}$ is the process noise matrix, and $\textbf{G}$ is the noise input matrix.
% For simplicity, $\textbf{G}=\textbf{I}$.
% It is also assumed that Agent 0 is perfectly aware of its own orientation $\textbf{R}$.
% The goal is now for Agent 0 to autonomously track and monitor Agents $1,\dots,n$ by minimizing the state uncertainty of every agent in the system.

% \subsection{Constraints}

% \subsubsection{Kinematic and Dynamic Constraints}
% Must follow physics, Decide on attitude parameterization set

% \subsubsection{Boundary Constraints}
% Control Torque Bounds, Angular Velocity Bounds, Uncertainty Bounds

% \subsubsection{Pointing Exclusion Zones}
% Don't point at sun
\end{comment}
